The Symbiotic X-ray binaries Sct X-1, 4U 1700+24 and IGR J17329-2731

Symbiotic X-ray binaries are systems hosting a neutron star accreting form the wind of a late type companion. These are rare objects and so far only a handful of them are known. One of the most puzzling aspects of the symbiotic X-ray binaries is the possibility that they contain strongly magnetized neutron stars. These are expected to be evolutionary much younger compared to their evolved companions and could thus be formed through the (yet poorly known) accretion induced collapse of a white dwarf. In this paper, we perform a broad-band X-ray and soft $\gamma$-ray spectroscopy of two known symbiotic binaries, Sct X-1 and 4U 1700+24, looking for the presence of cyclotron scattering features that could confirm the presence of strongly magnetized NSs. We exploited available Chandra, Swift, and NuSTAR data. We find no evidence of cyclotron resonant scattering features (CRSFs) in the case of Sct X-1 but in the case of 4U 1700+24 we suggest the presence of a possible CRSF at $\sim$16 keV and its first harmonic at $\sim$31 keV, although we could not exclude alternative spectral models for the broad-band fit. If confirmed by future observations, 4U 1700+24 could be the second symbiotic X-ray binary with a highly magnetized accretor. We also report about our long-term monitoring of the last discovered symbiotic X-ray binary IGR J17329-2731 performed with Swift/XRT. The monitoring revealed that, as predicted, in 2017 this object became a persistent and variable source, showing X-ray flares lasting for a few days and intriguing obscuration events that are interpreted in the context of clumpy wind accretion.

==> u1700_xrtlog_ordered.tex <==
%%%%%%%%  Fri Feb 25 14:09:47 CET 2022
%%%%%%%%  Wed Feb 23 12:07:27 CET 2022
%%%%%%%% Sat Feb 19 16:03:22 CET 2022
%%%%%%%% Fri Feb 18 17:04:30 CET 2022  
%%%%%%%% Wed Jan 26 13:38:00 CET 2022
%%%%%%%% Wed Jan 26 13:38:00 CET 2022
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% caldbmis.txt   /usr/local/caldb-6.28/data/swift/mis/caldb.indx -> index/caldb.indx20211105 
% caldbxrt.txt   /usr/local/caldb-6.28/data/swift/xrt/caldb.indx -> index/caldb.indx20210915 
% fversion       04Aug2021_V6.29b 
% swiftversion   Swift_Rel5.5(Bld44)_15Jul2021 
% xrtversion     swxrtdas_03May21_v3.6.1  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%
 %\setcounter{table}{0}		
\begin{table*} 	
 \begin{center} 	
 \caption{ 
{\it Swift}/XRT observation log of \srcc: observing sequence, date (MJD of the middle of the observation), start and end times (UTC), 
 XRT exposure time, and time since each BAT trigger for the start of the observation. 
%{\color{ballblue} PLACEHOLDER} 
}	
 \label{u1700:tab:swift_xrt_log} 	
 \begin{tabular}{ lllll l } 
 \hline 
 \hline 
 \noalign{\smallskip} 
  Sequence   & MJD  & Start time  (UT)                 & End time   (UT)        & Exposure  & Time since trigger\\ 
                    &          &(yyyy-mm-dd hh:mm:ss)  & (yyyy-mm-dd hh:mm:ss)  &(s)   &(s)               \\
 \noalign{\smallskip} 
 \hline 
 \noalign{\smallskip} 
%
%
%00090480001	&	55346.91980	&	2010-05-30 20:29:05	&	2010-05-30 23:39:55	&	1457 &	\\  %PC
%00090480002	&	55351.77498	&	2010-06-04 12:54:59	&	2010-06-05 00:16:57	&	9768 &	\\ %PC
%
%
%00540255000	&	56263.38193	&	2012-12-02 05:07:33	&	2012-12-02 13:12:24	&	12895 &	\\ %PC
%00540255000	&	56263.38026	&	2012-12-02 05:07:20	&	2012-12-02 13:07:49	&	27 &	\\ % WT 
%00540255001	&	56263.75986	&	2012-12-02 13:13:56	&	2012-12-02 23:14:27	&	6466 &	\\%PC
%00540255002	&	56264.79179	&	2012-12-03 14:56:26	&	2012-12-03 23:03:54	&	5300 &	\\%PC
%00540255003	&	56265.23469	&	2012-12-04 00:47:17	&	2012-12-04 10:28:36	&	5877 &	\\%PC
%00540255004	&	56266.65740	&	2012-12-05 13:21:41	&	2012-12-05 18:11:36	&	5980 &	\\%PC
%
% 
00612974000 BAT&	56917.56773   & 2014-09-17 13:28:15 &      2014-09-17 13:46:48     &     1113  & $-$150  \\ %TRIGTIME MET 432653448
00612974000 WT &	56917.63500	& 2014-09-17 13:50:28	&	2014-09-17 16:38:20	&	629	 &  1183  \\% WT 
%%00612974000$^{\mathrm{a}}$ PC  &	56917.66003	& 2014-09-17 14:57:58	&	2014-09-17 16:42:55	&	1484 & 5233	\\ %PC
%
% 00612974001	&	56917.89122	&	2014-09-17 16:46:16	&	2014-09-18 02:00:29	&	1605 &  11731	\\% WT 
% 00612974001	&	56917.87154	&	2014-09-17 16:46:50	&	2014-09-18 01:03:12	&	1848 &  11766	\\        %PC
% 00612974003	&	56919.82257	&	2014-09-18 16:38:02	&	2014-09-20 22:50:58	&	4004 &  97638	\\% WT 
% 00612974002	&	56919.49659	&	2014-09-19 11:41:13	&	2014-09-19 12:08:58	&	1665 & 166228	\\% WT 
% 00612974005	&	56921.43709	&	2014-09-21 07:10:50	&	2014-09-21 13:48:00	&	1997 & 322805	\\% WT 
% 00612974006	&	56922.15721	&	2014-09-22 01:55:50	&	2014-09-22 05:36:58	&	2052 & 390306	\\% WT 
% 00612974007	&	56923.53012	&	2014-09-23 03:41:50	&	2014-09-23 21:44:57	&	719	 &  483065    \\% WT 
% 00612974008	&	56924.35535	&	2014-09-24 06:42:31	&	2014-09-24 10:20:58	&	1992 & 580306	\\% WT 
% 00612974009	&	56925.91510	&	2014-09-25 21:03:35	&	2014-09-25 22:51:58	&	1792 &	718371 \\% WT 
% 00612974010	&	56926.82556	&	2014-09-26 19:34:38	&	2014-09-26 20:02:58	&	1699 &	799433	\\% WT 
% 00612974012	&	56928.44427	&	2014-09-28 09:50:31	&	2014-09-28 11:29:00	&	1741 &	937187	\\% WT 
% 00612974013	&	56929.15161	&	2014-09-29 03:24:41	&	2014-09-29 03:51:58	&	1635 &	1000437	\\% WT 
% 00612974014	&	56930.21695	&	2014-09-30 04:57:52	&	2014-09-30 05:26:58	&	1745 &	1092427	\\% WT 
% 00612974015	&	56931.88274	&	2014-10-01 20:57:24	&	2014-10-01 21:24:58	&	1650 &	1236399	\\        % WT 
% %%00080848001&	56932.91507	&	2014-10-02 21:04:10	&	2014-10-02 22:51:14	&	105	  &	1323206      \\ % WT 
% 00080848001      &	56932.92032	&	2014-10-02 21:05:35	&	2014-10-02 23:04:55	&	1921 &	1323290	\\        % PC 
% 00612974017	&	56935.08039	&	2014-10-05 01:46:56	&	2014-10-05 02:04:58	&	1060 &	1512971	\\% WT 
% 00612974018	&	56937.28486	&	2014-10-07 06:45:44	&	2014-10-07 06:54:39	&	534	  & 	1703700     \\% WT 
% 00612974019	&	56939.07336	&	2014-10-09 01:37:18	&	2014-10-09 01:53:58	&	999	 & 	1857993      \\% WT 
% 00612974020	&	56941.61684	&	2014-10-11 14:39:35	&	2014-10-11 14:56:58	&	1040 &	2077730	\\% WT 
% 00612974021	&	56943.40283	&	2014-10-13 09:31:12	&	2014-10-13 09:48:58	&	1065 &	2232027	\\% WT 
% 00612974022	&	56945.20259	&	2014-10-15 04:43:34	&	2014-10-15 04:59:58	&	980    & 	2387569 	\\% WT 
% 00612974023	&	56947.47774	&	2014-10-17 11:18:59	&	2014-10-17 11:36:58	&	1075 &	2584094	\\% WT 
% 00612974024	&	56949.07922	&	2014-10-19 01:45:12	&	2014-10-19 02:02:58	&	1065 &	2722468	\\% WT 
% 00612974025	&	56951.34428	&	2014-10-21 08:06:42	&	2014-10-21 08:24:58	&	1087 &	2918158	\\% WT 
% 00612974026	&	56953.75738	&	2014-10-23 17:20:17	&	2014-10-23 19:00:58	&	980	  &	3124173      \\% WT 
% 00612974027	&	56955.12684	&	2014-10-25 02:53:24	&	2014-10-25 03:11:58	&	1110 &	3244959	\\% WT 
% 00612974028	&	56957.12662	&	2014-10-27 02:53:42	&	2014-10-27 03:10:58	&	1035 &	3417778	\\% WT 
% 00612974029	&	56959.12356	&	2014-10-29 02:51:15	&	2014-10-29 03:04:39	&	800	  &	3590431      \\% WT 
% 00612974030 	&	56961.53602	&	2014-10-31 12:43:47	&	2014-10-31 12:59:58	&	970	  &	3798782      \\% WT 
\noalign{\smallskip}
%
% trigger 3 
00621278000 BAT	&     57004.15625   &      2014-12-13 01:52:22     &     2014-12-13 05:37:37     &      13516 &  $-$239	\\ %TRIGTIME MET   440128584
00621278000 WT	&	57004.17946	&	2014-12-13 01:58:20	&	2014-12-13 06:38:33	&	2002 & 120	\\% WT 
%00621278000$^{\mathrm{a}}$ PC	&	57004.18396	&	2014-12-13 03:15:51	&	2014-12-13 05:33:57	&	5045 & 4770	\\% PC 
 \noalign{\smallskip}
% trigger 4
00623434000 BAT      &     57026.72587    &     2015-01-04 15:35:18	&     2015-01-04 19:12:02     &     13195 & $-$239 \\ %TRIGTIME MET  442078760
00623434000 WT	&	57026.72471	&	2015-01-04 15:46:02	&	2015-01-04 19:01:06	&	4656 & 406	\\% WT 
%00623434000$^{\mathrm{a}}$ PC 	&	57026.76695	&	2015-01-04 17:36:50	&	2015-01-04 19:11:57	&	1161 & 7054	\\% PC 
 \noalign{\smallskip}
  \hline
  \end{tabular}
  \end{center}
 % \begin{list}{}{} 
 %\item[$^{\mathrm{a}}$] BAT trigger on \srcc.
%\end{list} 
  \end{table*} 

